Edge-featured Graph Neural Architecture Search

Graph neural networks (GNNs) have been successfully applied to learning representation on graphs in many relational tasks. Recently, researchers study neural architecture search (NAS) to reduce the dependence of human expertise and explore better GNN architectures, but they over-emphasize entity features and ignore latent relation information concealed in the edges. To solve this problem, we incorporate edge features into graph search space and propose Edge-featured Graph Neural Architecture Search to find the optimal GNN architecture. Specifically, we design rich entity and edge updating operations to learn high-order representations, which convey more generic message passing mechanisms. Moreover, the architecture topology in our search space allows to explore complex feature dependence of both entities and edges, which can be efficiently optimized by differentiable search strategy. Experiments at three graph tasks on six datasets show EGNAS can search better GNNs with higher performance than current state-of-the-art human-designed and searched-based GNNs.

==> checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} See Section Boarder Impact. 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} We think there are no negative societal impacts. 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{} 
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} See supplementary materials. 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See Section~\ref{exp}. 
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} See Table~\ref{tab_graph}, Table~\ref{tab_ZINC_TSP} and Table~\ref{tab_node}. 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See Section~\ref{gpu}, Table~\ref{tab_graph}, Table~\ref{tab_ZINC_TSP} and Table~\ref{tab_node}. 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} See references. 
  \item Did you mention the license of the assets?
    \answerYes{} They use MIT license. 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} See supplemental materials. 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} 
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{} 
\end{enumerate}

\end{enumerate}

==> table.tex <==
\begin{table}[t]
    \small
    \centering
    \setlength{\tabcolsep}{0.7 mm}
    \begin{tabular}{@{}l|c|ccc|ccc|ccc@{}}
    \toprule
                                            &          & \multicolumn{3}{c|}{{SBM-CLUSTER}}         & \multicolumn{3}{c|}{{TSP}}                 & \multicolumn{3}{c}{{ZINC}}              \\
    {Architecture}                          & {Search} & {Params}    & {Test Acc.}     & {Search}   & {Params}    & {Test Acc.}    & {Search}    & {Params}    & {Test MAE.}    & {Search} \\
                                            & {Method} & ({M})       & (\%)            & {Cost}     & ({M})       & (\%)           & {Cost}      & ({M})       & (MAE)          & {Cost}   \\
    \midrule
    GCN~\cite{kipf2016semi}                 & manual   & 0.50        & 68.5            & -          & 0.50        & 71.9           & -           & 0.50        & 68.5           & -      \\
    GIN~\cite{xu2018powerful}               & manual   & 0.51        & 64.7            & -          & 0.51        & 85.4           & -           & 0.52        & 64.7           & -      \\
    GraphSage~\cite{hamilton2017inductive}  & manual   & 0.50        & 63.8            & -          & 0.50        & 50.5           & -           & 0.53        & 63.8           & -      \\
    GAT~\cite{velivckovic2017graph}         & manual   & 0.53        & 70.6            & -          & 0.53        & 78.3           & -           & 0.53        & 70.6           & -      \\
    GatedGCN (E)~\cite{bresson2017residual} & manual   & 0.50        & 76.1            & -          & 0.50        & 86.5           & -           & 0.53        & 76.0           & -      \\
    GNAS-RL~\cite{gao2020graph}             & RL       & -           & -               & -          & -           & -              & -           & -           & -              & -      \\
    GNAS-MP~\cite{cai2021rethinking}        & gradient & 1.60        & 74.8            & 3.21h      & -           & -              & -           & -           & -              & -      \\
    \midrule 
    EF-GNAS (wo E)                          & gradient & -           & -               & -          & -           & -              & -           & -           & -              & -      \\
    EF-GNAS (E)                             & gradient & -           & -               & -          & -           & -              & -           & -           & -              & -      \\
    \bottomrule
    \end{tabular}
\end{table}
